Tree-level invariants of three-manifolds, Massey products and the Johnson homomorphism

Two references added and the introduction slightly expanded. We show that the tree-level part of a recent theory of invariants of 3-manifolds (due, independently, to Goussarov and Habiro) is essentially given by classical algebraic topology in terms of the Johnson homomorphism and Massey products, for arbitrary 3-manifolds. A key role of our proof is played by the notion of a homology cylinder, viewed as an enlargement of the mapping class group, and an apparently new Lie algebra of graphs colored by the first homology of a closed surface, closely related to deformation quantization on a surface as well as to a Lie algebra that encodes the symmetries of Massey products and the Johnson homomorphism. In addition, we present a realization theorem for Massey products and the Johnson homomorphism on homology cylinders.

==> draws/Y1.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(3773,1186)(0,-10)
\thicklines
\path(312,859)(612,559)(312,259)
\path(612,559)(1212,559)
\drawline(12,1159)(12,1159)
\path(1512,1009)(1512,559)
\path(1512,334)(1512,34)
\path(1437,709)	(1378.882,690.556)
	(1330.652,672.903)
	(1261.219,638.215)
	(1223.426,601.419)
	(1212.000,559.000)

\path(1212,559)	(1238.006,503.528)
	(1300.099,460.450)
	(1374.392,429.147)
	(1437.000,409.000)

\path(1437,409)	(1470.588,402.852)
	(1512.000,400.802)
	(1553.412,402.852)
	(1587.000,409.000)

\path(1587,409)	(1649.608,429.147)
	(1723.901,460.450)
	(1785.994,503.528)
	(1812.000,559.000)

\path(1812,559)	(1800.574,601.425)
	(1762.781,638.223)
	(1693.348,672.909)
	(1645.118,690.559)
	(1587.000,709.000)

\path(3461,858)(3161,558)(3461,258)
\path(3161,558)(2561,558)
\drawline(3761,1158)(3761,1158)
\path(2261,1008)(2261,558)
\path(2261,333)(2261,33)
\path(2336,708)	(2394.118,689.556)
	(2442.348,671.903)
	(2511.781,637.215)
	(2549.574,600.419)
	(2561.000,558.000)

\path(2561,558)	(2534.994,502.528)
	(2472.901,459.450)
	(2398.608,428.147)
	(2336.000,408.000)

\path(2336,408)	(2302.412,401.852)
	(2261.000,399.802)
	(2219.588,401.852)
	(2186.000,408.000)

\path(2186,408)	(2123.392,428.147)
	(2049.099,459.450)
	(1987.006,502.528)
	(1961.000,558.000)

\path(1961,558)	(1972.426,600.425)
	(2010.219,637.223)
	(2079.652,671.909)
	(2127.882,689.559)
	(2186.000,708.000)

\put(1887.000,671.500){\arc{375.000}{3.7851}{5.6397}}
\drawline(1662,559)(1662,559)
\path(1662,559)(1662,634)
\path(2112,634)(2112,559)
\path(1662,559)	(1731.819,488.102)
	(1789.076,441.812)
	(1839.045,416.617)
	(1887.000,409.000)

\path(1887,409)	(1934.955,416.617)
	(1984.924,441.812)
	(2042.181,488.102)
	(2112.000,559.000)

\end{picture}


==> draws/Y10.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1566,510)(0,-10)
\thicklines
\path(1233,333)(1533,483)
\path(33,33)(1533,33)
\path(33,333)(1233,333)(1533,183)
\end{picture}


==> draws/Y2.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(3773,1186)(0,-10)
\thicklines
\path(312,859)(612,559)(312,259)
\path(612,559)(1212,559)
\drawline(12,1159)(12,1159)
\path(1512,1009)(1512,559)
\path(1512,334)(1512,34)
\path(1437,709)	(1378.882,690.556)
	(1330.652,672.903)
	(1261.219,638.215)
	(1223.426,601.419)
	(1212.000,559.000)

\path(1212,559)	(1238.006,503.528)
	(1300.099,460.450)
	(1374.392,429.147)
	(1437.000,409.000)

\path(1437,409)	(1470.588,402.852)
	(1512.000,400.802)
	(1553.412,402.852)
	(1587.000,409.000)

\path(1587,409)	(1649.608,429.147)
	(1723.901,460.450)
	(1785.994,503.528)
	(1812.000,559.000)

\path(1812,559)	(1800.574,601.425)
	(1762.781,638.223)
	(1693.348,672.909)
	(1645.118,690.559)
	(1587.000,709.000)

\path(3461,858)(3161,558)(3461,258)
\path(3161,558)(2561,558)
\drawline(3761,1158)(3761,1158)
\path(2261,1008)(2261,558)
\path(2261,333)(2261,33)
\path(2336,708)	(2394.118,689.556)
	(2442.348,671.903)
	(2511.781,637.215)
	(2549.574,600.419)
	(2561.000,558.000)

\path(2561,558)	(2534.994,502.528)
	(2472.901,459.450)
	(2398.608,428.147)
	(2336.000,408.000)

\path(2336,408)	(2302.412,401.852)
	(2261.000,399.802)
	(2219.588,401.852)
	(2186.000,408.000)

\path(2186,408)	(2123.392,428.147)
	(2049.099,459.450)
	(1987.006,502.528)
	(1961.000,558.000)

\path(1961,558)	(1972.426,600.425)
	(2010.219,637.223)
	(2079.652,671.909)
	(2127.882,689.559)
	(2186.000,708.000)

\end{picture}


==> draws/Y3.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(3773,1185)(0,-10)
\thicklines
\path(312,858)(612,558)(312,258)
\path(612,558)(1212,558)
\drawline(12,1158)(12,1158)
\path(3461,857)(3161,557)(3461,257)
\path(3161,557)(2561,557)
\drawline(3761,1157)(3761,1157)
\path(1212,558)(2562,558)
\path(1512,1083)(1512,633)
\path(2262,1083)(2262,633)
\path(1512,483)(1512,33)
\path(2262,483)(2262,33)
\end{picture}


==> draws/Y4.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1520,1056)(0,-10)
\thicklines
\path(12,858)(312,558)(12,258)
\path(312,558)(912,558)
\path(1062,1008)(1062,558)
\path(1362,1008)(1362,558)
\path(1062,333)(1062,33)
\path(1362,333)(1362,33)
\path(1137,633)(1287,633)
\path(987,633)	(928.406,597.611)
	(912.000,558.000)

\path(912,558)	(941.295,510.101)
	(987.000,483.000)

\path(987,483)	(1034.260,458.524)
	(1095.079,434.160)
	(1158.108,415.466)
	(1212.000,408.000)

\path(1212,408)	(1265.892,415.466)
	(1328.921,434.160)
	(1389.740,458.524)
	(1437.000,483.000)

\path(1437,483)	(1482.705,510.101)
	(1512.000,558.000)

\path(1512,558)	(1495.594,597.611)
	(1437.000,633.000)

\end{picture}


==> draws/Y5.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1394,1057)(0,-10)
\thicklines
\put(986.000,559.000){\arc{150.000}{1.5708}{4.7124}}
\put(1136.000,559.000){\arc{150.000}{4.7124}{7.8540}}
\path(12,858)(312,558)(12,258)
\path(312,558)(912,558)
\path(1062,1008)(1062,558)
\path(1062,333)(1062,33)
\path(986,484)(1136,484)
\path(1361,1009)(1361,34)
\end{picture}


==> draws/Y6.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1520,1057)(0,-10)
\thicklines
\put(1436.000,559.000){\arc{150.000}{4.7124}{7.8540}}
\put(1286.000,559.000){\arc{150.000}{1.5708}{4.7124}}
\path(12,858)(312,558)(12,258)
\path(312,558)(912,558)
\path(1362,1008)(1362,558)
\path(1362,333)(1362,33)
\path(1286,484)(1436,484)
\path(911,559)(1211,559)
\path(1061,1009)(1061,634)
\path(1061,334)(1061,34)
\end{picture}


==> draws/Y7.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(3173,1131)(0,-10)
\thicklines
\put(1962,558){\ellipse{600}{300}}
\put(1587,558){\ellipse{600}{300}}
\put(1212,558){\ellipse{600}{300}}
\path(12,858)(312,558)(12,258)
\path(312,558)(912,558)
\path(3161,857)(2861,557)(3161,257)
\path(2861,557)(2261,557)
\path(1212,1083)(1212,783)
\path(1212,333)(1212,33)
\path(1962,333)(1962,33)
\path(1212,633)(1212,483)
\path(1962,633)(1962,483)
\path(1962,1083)(1962,783)
\end{picture}


==> draws/Y8.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(3173,1131)(0,-10)
\thicklines
\path(12,858)(312,558)(12,258)
\path(312,558)(912,558)
\path(3161,857)(2861,557)(3161,257)
\path(2861,557)(2261,557)
\path(1212,1083)(1212,783)
\path(1212,333)(1212,33)
\path(1962,333)(1962,33)
\path(1962,1083)(1962,783)
\path(912,558)(2262,558)
\end{picture}


==> draws/Y9.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(1566,820)(0,-10)
\thicklines
\path(1158,418)(1233,643)(1533,493)
\path(1233,643)(1533,793)
\path(33,343)(408,343)
\path(558,343)(1533,343)
\path(33,643)	(91.026,655.029)
	(141.429,663.621)
	(185.089,668.777)
	(222.885,670.495)
	(284.398,663.621)
	(333.000,643.000)

\path(333,643)	(389.417,590.318)
	(429.620,518.507)
	(445.329,477.420)
	(459.012,433.942)
	(471.344,388.869)
	(483.000,343.000)
	(494.656,297.131)
	(506.988,252.058)
	(520.671,208.580)
	(536.380,167.493)
	(576.583,95.682)
	(633.000,43.000)

\path(633,43)	(702.351,16.548)
	(742.256,10.588)
	(783.611,9.122)
	(824.890,11.892)
	(864.566,18.635)
	(933.000,43.000)

\path(933,43)	(1005.090,113.241)
	(1041.560,177.419)
	(1061.439,219.080)
	(1083.000,268.000)

\end{picture}


==> draws/g0.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(1224,629)(0,-10)
\put(612,307){\ellipse{1200}{600}}
\path(12,307)(1212,307)
\end{picture}
}


==> draws/g2.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(1224,569)(0,-10)
\put(612,277){\ellipse{540}{540}}
\path(12,277)(312,277)
\path(912,277)(1212,277)
\end{picture}
}


==> draws/g4.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(1224,639)(0,-10)
\path(12,612)(312,312)(12,12)
\path(312,312)(912,312)
\path(1212,612)(912,312)(1212,12)
\end{picture}
}


==> draws/lie.tex <==
%\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(9491,1231)(0,-10)
\thicklines
\path(1245.000,514.000)(1125.000,484.000)(1245.000,454.000)
\put(1125.000,634.000){\arc{300.000}{4.7124}{7.8540}}
\path(405.000,454.000)(525.000,484.000)(405.000,514.000)
\put(525.000,634.000){\arc{300.000}{1.5708}{4.7124}}
\path(5806.000,453.000)(5926.000,483.000)(5806.000,513.000)
\put(5926.000,633.000){\arc{300.000}{1.5708}{4.7124}}
\path(225,934)(525,634)(1125,634)(1425,934)
\path(225,334)(525,634)
\path(1125,634)(1425,334)
\path(2025,634)(2625,634)
\path(2505.000,604.000)(2625.000,634.000)(2505.000,664.000)
\path(5626,933)(5926,633)(6226,933)
\path(5926,633)(5926,333)
\path(6826,633)(7426,633)
\path(7306.000,603.000)(7426.000,633.000)(7306.000,663.000)
\put(75,34){\makebox(0,0)[lb]{$c$}}
\put(1275,34){\makebox(0,0)[lb]{$b$}}
\put(0,1084){\makebox(0,0)[lb]{$\ast$}}
\put(1275,1084){\makebox(0,0)[lb]{$a$}}
\put(3075,559){\makebox(0,0)[lb]{$[c,[a,b]]$}}
\put(5326,1083){\makebox(0,0)[lb]{$a$}}
\put(6301,1083){\makebox(0,0)[lb]{$b$}}
\put(5776,33){\makebox(0,0)[lb]{$c$}}
\put(7876,558){\makebox(0,0)[lb]{$a \otimes [c,b]+ c\otimes[b,a] +
b\otimes [a,c]$}}
\end{picture}

